Fast Bayesian Coresets via Subsampling and Quasi-Newton Refinement

Bayesian coresets approximate a posterior distribution by building a small weighted subset of the data points. Any inference procedure that is too computationally expensive to be run on the full posterior can instead be run inexpensively on the coreset, with results that approximate those on the full data. However, current approaches are limited by either a significant run-time or the need for the user to specify a low-cost approximation to the full posterior. We propose a Bayesian coreset construction algorithm that first selects a uniformly random subset of data, and then optimizes the weights using a novel quasi-Newton method. Our algorithm is a simple to implement, black-box method, that does not require the user to specify a low-cost posterior approximation. It is the first to come with a general high-probability bound on the KL divergence of the output coreset posterior. Experiments demonstrate that our method provides significant improvements in coreset quality against alternatives with comparable construction times, with far less storage cost and user input required.

==> theory.tex <==
\section{Theoretical Analysis}\label{sec:theory}

In this section we provide a theoretical analysis of the proposed method.
First, we demonstrate (in \cref{thm:optimal_kl}) that the 
optimal coreset posterior built using a uniformly random subset of data
is, with high probability, a good approximation of the true posterior---and in some cases is \emph{exact}.
Second, we show (in \cref{thm:convergence}) that the proposed optimization algorithm converges 
exponentially quickly to a point near the optimal coreset, thus realizing 
the guarantee in \cref{thm:optimal_kl} in practice.
Proofs of all results may be found in \cref{sec:proofs}.

\subsection{Subset selection via uniform subsampling}\label{sec:theory-sel}
\cref{thm:optimal_kl} provides a theoretical foundation for the selection via
uniform subsampling. It makes two assertions. First, in a
general setting, with high probability the optimal coreset using a uniformly
random selection of data provides low error. Second, when the log likelihood
functions are actually finite-dimensional, with high probability the optimal
coreset using a uniformly random selection of data is exact. 
After the statement of \cref{thm:optimal_kl}, we provide intuition
on its major components and walk through a representative example application
that demonstrates that the optimal KL divergence stays roughly constant despite
an increasing dataset size $N$. Therefore, as long as one has a reliable
method to optimize the weights, uniformly randomly selecting the data 
points is not limiting.

In what follows, we assume that the functions $f_n(\cdot)$ are generated i.i.d.,
$f_n(\cdot) \overset{\text{i.i.d.}}{\sim} p$,
from some true data-generating distribution $p$. For example, in the typical frequentist setup, 
$f_n(\cdot) = \log \ell(X_n | \cdot)$ 
for $X_n \overset{\text{i.i.d.}}{\sim} p_{\theta_0}$. 
Let $C$ be the universal constant in \citet[Corollary 1.2]{Boroczky03},
and for $d\in\mathbb{N}$, let $A_d = e^{\frac{d}{2}}d^{\frac{3}{2}}\log(1+d)$.
Finally, let the functions $F$, $U$, $V$, and $J$ be as 
defined in Eqs.~(\ref{eq:thm1_J}-\ref{eq:thm1_U}).
\begin{theorem}\label{thm:optimal_kl}
Let $\mu$ be a probability measure on $\Theta$ such that 
$\mathbb{E}\left[f_1^2(\theta)\right] < \infty$ for $\theta\sim\mu$ and $f_1(\cdot)\sim p$. Define $M\in[N]$,
$d\in\mathbb{N}$, 
and a $d$-dimensional subspace $S$ of $L^2(\mu)$ with orthogonal complement $S_\perp$.
Then we have the following two results:
\begin{enumerate}
\item For any $t,s,r>0$ and 
$\phi \in \left(0, \arccos\frac{1}{\sqrt{d+1}}\right]$, 
 with probability at least 
\begin{align*}
 1 - J(t) - V(s) - U(r)^M - C A_d \phi^{-d}F(\phi, 0)^M,
\end{align*}
we have that
\begin{align*}
\min_{w\in\mathcal{W}_N}\mathrm{KL}(\pi_{w}||\pi) &\leq N^2t(s+r)^2.
\end{align*}
\item If $S_\perp = \emptyset$, for any $t,s>0$ and
$\phi \in \left(0, \arccos\frac{1}{\sqrt{d+1}}\right]$, 
with probability at least
\begin{align*}
1 - J(t) - V(s) - C A_d \phi^{-d}F(\phi, s)^M,
\end{align*}
we have that
\begin{align*}
\min_{w\in\mathcal{W}_N}\mathrm{KL}(\pi_{w}||\pi) &= 0.
\end{align*}
\end{enumerate}
\end{theorem}

Note that since $\mathcal{W}_N \subset \mathcal{W}$, 
\cref{thm:optimal_kl} also bounds $\min_{w\in\mathcal{W}} \mathrm{KL}(\pi_w||\pi)$.
In order to use \cref{thm:optimal_kl} for a particular application of interest, 
you need to pick a distribution $\mu$ and a subspace $S$ of $L^2(\mu)$, 
and then obtain upper bounds on the functions $J(t)$, $V(s)$, $U(r)$, and $F(\phi,u)$ 
defined in Eqs.~(\ref{eq:thm1_J}-\ref{eq:thm1_U}).
In the following we provide more details and intuition for each step, 
as well as defining the relevant functions appearing in \cref{thm:optimal_kl}.
To illustrate each step in practice, we will demonstrate
the application of Statement 1.~of \cref{thm:optimal_kl} to
a Bayesian Gaussian location model in $\mathbb{R}^d$
\begin{align*}
\theta &\sim \mathcal{N}(0, I), \quad \theta\in\mathbb{R}^d\\
X_n &\overset{\text{i.i.d.}}{\sim} \mathcal{N}(\theta, I), \quad X_n\in\mathbb{R}^d,
\end{align*}
where the data $X_n$ are truly generated via
$X_n \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, I)$.
Note that while this running example model is well-specified, 
it is not a requirement of the theory.

\paragraph{Step 1a: Pick a surrogate distribution.}
The first step is to select a fixed probability measure $\mu$ on $\Theta$
such that $\mathbb{E}\left[f_1^2(\theta)\right] < \infty$ (under both $\theta \sim \mu$ and $f_1 \sim p$).
Intuitively, $\mu$ should place mass in the region roughly where the posterior concentrates
as $N\to\infty$.

In our running example, we set $\mu = \mathcal{N}(0, I)$.
Since the log-likelihood functions here are quadratic in both $X_n$ and $\theta$,
and both $\mu$ and $p$ are Gaussian, the finite expectation requirement is satisfied.

\paragraph{Step 1b: Bound relative difference with KL.}
In the proof of the result, we replace the KL divergence with 
the squared $L^2(\mu)$ norm and analyze the error in that space instead. 
Doing this makes the problem more tractable. However, 
we do need to bound the relative error that we incur 
by working with the $L^2(\mu)$ norm rather than with the KL divergence directly.
In other words,
we require a bound on the probability
\begin{align}\label{eq:thm1_J}
J(t) &= \Pr\left(\max_{m\in[M]}\sup_{w\in\mathcal{W}_N}R(w,m)  > t\right),
\end{align}
where for notational brevity we define
\begin{align*}
Y(t, m) &= \int_0^1(1-t)\mathrm{Cov}_{\pi_{(1-t)N1_m+t1}}\left(f(\theta)\right)\mathrm{d}t\\
R(w,m) &= \frac{(1-w)^TY(t,m)(1-w)}{(1-w)^T\mathrm{Cov}_{\mu}\left(f(\theta)\right)(1-w)}.
\end{align*}
In our running example, we have that for distribution $\mu$,
\begin{align*}
\mathrm{Cov}_{\mu}\left(f_i(\theta), f_j(\theta)\right) = \frac{d}{2} + X_i^TX_j,
\end{align*}
and so for any $w\in\mathcal{W}_N$,
{\small
\begin{align*}
(1-w)^T\mathrm{Cov}_{\mu}\left(f(\theta)\right)(1-w) = \left\|\sum_n X_n - \sum_n w_nX_n\right\|^2.
\end{align*}
}
Similar algebra (see \cref{sec:example}) yields
{\small
\begin{align*}
(1-w)^TY(t,m)(1-w) = \frac{1}{1+N}\left\|\sum_n X_n - \sum_n w_nX_n\right\|^2.
\end{align*}
}%
Therefore for $w\in\mathcal{W}_N$, $m\in[M]$, $R(w,m) = (1+N)^{-1}$.

\paragraph{Step 2: Bound the scale of the problem.}
From this point onward, we are able to work entirely in $L^2(\mu)$.
Define the vector $f_n\in L^2(\mu)$ corresponding to the function
$f_n(\theta) - \mathbb{E}_\mu\left[f_n(\theta)\right]$, i.e., the log-likelihood
function for data point $n$ shifted by its expectation under $\mu$.
Also define the expectation of the vector $f_n$ under the data-generating distribution,
$\bar f = \mathbb{E}\left[f_1\right]$.
In our running example,
\begin{align}
\begin{aligned}
f_n(\theta) - \mathbb{E}_\mu\left[f_n(\theta)\right] &= X_n^T\theta +\frac{1}{2}(d-\|\theta\|^2)\\
\bar f(\theta) &= \frac{1}{2}(d-\|\theta\|^2)\\
\left<f_n-\bar f, f_m-\bar f\right>_{L^2(\mu)} &= X_n^TX_m.
\end{aligned}\label{eq:example_inner_prod}
\end{align}

The next task is to bound the scale of the approximation problem
via the tail probability
\begin{align}\label{eq:thm1_V}
V(s) &= \Pr\left( \left\|\frac{1}{N}\sum_{n=1}^Nf_n-\bar f \right\| > s\right).
\end{align}
Note that in \cref{eq:thm1_V}, 
we deal with the empirical average $\frac{1}{N}\sum_n f_n$; the factor
of $N^2$ appearing in Statement 1.~of \cref{thm:optimal_kl} comes from
making this switch from sum to average.

In our running example, \cref{eq:example_inner_prod} implies that
$\left\|\frac{1}{N}\sum_n f_n - \bar f\right\|^2 = \left\|\frac{1}{N}\sum_n X_n\right\|^2$.
Further, $\left\|\frac{1}{\sqrt{N}}\sum_{n=1}^NX_n\right\|^2$ has a $\chi^2$ distribution
with $d$ degrees of freedom. So therefore
\begin{align*}
V(s) &\leq e^{d/2 - (Ns^2/2) + (d/2)\log (Ns^2/d)}.
\end{align*}


\paragraph{Step 3a: Split $L^2(\mu)$ into two subspaces.}
Typically, the full $L^2(\mu)$ space will be infinite dimensional.
However, recall that we are only working with functions of the form
$f_n(\theta) = \log \ell(X_n|\theta)$ sampled i.i.d.~from some data-generating distribution; 
these typically \emph{mostly} fall in a finite-dimensional subspace of $L^2(\mu)$.  
In other words, we expect there to be a $d$-dimensional subspace $S$ of $L^2(\mu)$, $d\in\mathbb{N}$,
in which the log-likelihood functions have the majority of their $L^2(\mu)$ norm.
In the orthogonal complement, $S_\perp$, we expect the norms to be small.
In essence, $d$ is the ``effective dimension'' of the space of log-likelihood functions
that we work with; this ``effective dimension'' may in general increase with $N$
as more $\log \ell(X_n|\theta)$ functions are generated.

In the running example, \cref{eq:example_inner_prod} shows that the functions $f_n$
are in an isometry with $X_n \in \mathbb{R}^d$; hence the functions are
$d$-dimensional, and $S_\perp$ is empty.

\paragraph{Step 3b: Bound the coreset expressiveness in $S$.}
Within the subspace $S$, we require that the selected vectors $f_1,\dots, f_M$
provide an expressive basis for approximation. Since the $f_n$ are generated
i.i.d., we can simplify the problem to asking for a bound on how likely
it is that $f_1-\bar f$ aligns with any unit vector $a\in S$,
\begin{align}\label{eq:thm1_F}
&F(\phi, u) =\notag\\
&\!\!\!\!\!\!\!\sup_{a\in S, \|a\|=1}\!\!\!\!\Pr\left(\left<a, \frac{f_1-\bar f}{\|f_1-\bar f\|_{S}}\right> < \phi + \frac{u}{\|f_1-\bar f\|_S}\right).
\end{align}
For intuition, consider the case where $u=\phi=0$. At one extreme, where $f_1-\bar f$ has an isotropic
distribution in $S$, the above probability is $1/2$ regardless of $a\in S$. 
At the other extreme, where $f_1-\bar f$ is nearly concentrated in one direction,
then the above probability is $\approx 1$ if we pick $a$ to be in the opposite direction.
Since we want $F(\phi,u)$ to be as small as possible in the statement of \cref{thm:optimal_kl}, 
the more uniformly distributed the direction of $f_1-\bar f$ is, the better
of a basis $f_1,\dots, f_M$ will be. 

In our running example, we set $u=0$ per the first statement of \cref{thm:optimal_kl}.
Since the functions $f_n$ are in isometry with $X_n$,
and $X_n$ is from an isotropic Gaussian, then the probability $F(\phi,0)$ 
is related to the fraction of surface area of the $d$-dimensional sphere
remaining after removing a hyperspherical cap of height $1-\phi$,
\begin{align*}
F(\phi, 0) &= \frac{1}{2} + O(\phi), \quad \phi\to 0.
\end{align*}

\paragraph{Step 3c: Bound the complement norm.} 
Finally, we need to bound the norm of the component of 
the vectors $f_n-\bar f$ in the ``discarded'' orthogonal complement $S_\perp$.
Once again because the $f_n$ are i.i.d., we can consider just 
bounding the tail probability for the first vector, 
\begin{align}\label{eq:thm1_U}
U(r) &= \Pr\left( \left\|f_1 - \bar f\right\|_{S_\perp} > r\right).
\end{align}

In our running example, $S_\perp = \emptyset$, so for any $r > 0$, we 
have that $U(r) = 0$.

\paragraph{Step 4: Combining the results.}
The last step is to combine the bounds on
$J(t)$, $V(s)$, $U(r)$, and $F(\phi, u)$
as in \cref{thm:optimal_kl}. 
In our running example,
if we select a coreset size of $M \propto d$,
then we can set
$t \propto 1/N$,
$s \propto 1/\sqrt{N}$,
$r \propto 1/N$, and $\phi \propto 2^{-M/d}$
in such a way that with constant probability,
\begin{align*}
\min_{w\in\mathcal{W}}\mathrm{KL}(\pi_w||\pi) = O(1) \quad \text{as}\quad N,d\to\infty.
\end{align*}
In other words, for this application, a reasonable subsample size for coreset construction scales linearly in size with the 
dimension of the space $d$, but otherwise provides a constant-size compression of the dataset in $N$.
Therefore, despite the generality of \cref{thm:optimal_kl}, it has recovered the ability to compress the data in
this model using sufficient statistics that do not grow as the dataset size $N$ grows. 
Note that the minimal sufficient statistic in this problem is $\sum_n X_n$, which has storage cost $O(d)$;
by using a weighted sparse data representation, the coreset has a storage cost of $O(d^2+d)$ for $O(d)$ vectors
in $\mathbb{R}^d$ and $d$ weights.

\subsection{Weight optimization via approximate Newton}\label{sec:theory-opt}
\cref{thm:optimal_kl} guarantees the existence of a high-quality coreset,
but does not provide any insight into whether it is possible to find it tractably. 
\cref{thm:convergence} addresses this remaining gap. 
In particular, intuitively, it asserts that as long as 
(1) the
regularization parameter $\tau>0$ is nonzero but small enough that it does
not interfere with the optimization (in particular, the minimum eigenvalue 
of $G(w)$ over the space), and
(2) the \emph{optimal} coreset is a good approximation to the full dataset
(which is already guaranteed by \cref{thm:optimal_kl}),
then
the weights $w_k$ at iteration $k$ of the approximate Newton method 
converge exponentially to a point close to a global optimum. 
In the result below, let $G(w)$ and $H(w)$ 
be defined as in \cref{eq:G_H_def}.

\begin{theorem}\label{thm:convergence}
Let $W\subseteq \mathcal{W}$ be a closed convex set,
$W^\star \subseteq \arg\!\min_{w\in W} \mathrm{KL}(\pi_w||\pi)$
be a maximal closed convex subset, and fix the regularization parameter $\tau > 0$.
Define
\begin{align*}
\xi = \inf_{w\in W} \min\left\{ \frac{\lambda}{\lambda+\tau} : \lambda \in \mathrm{eigvals}\,G(w), \, \lambda > 0\right\}.
\end{align*}
Suppose there exist $\epsilon\in [0,1)$ and $\delta \geq 0$ such that
for all $w\in W$ there exists $v\in\mathbb{R}^M$, $\|v\|\leq 1$ such that
\begin{align}
\hspace{-.3cm}\left(G(w)\!+\!\tau I\right)^{-1}H(w)(1\!-\!w^\star) &= (\epsilon \|w\!-\!w^\star\|\!+\!\delta) v, \label{eq:optw_error}
\end{align}
where $w^\star = \mathrm{proj}_{W^\star}(w)$.
Then the $k^\text{th}$ iterate $w_k\in W$ and its projection $w^\star_k = \mathrm{proj}_{W^\star}(w_k)$
of the projected Newton method 
initialized at $w_0\in W$ with step size $\gamma \in [0, 1]$
and with regularization $\tau$
satisfies
\begin{align*}
\left\|w_{k} - w^\star_k\right\|
&\leq \eta^{k}\left\|w_0 - w^\star_0\right\| + \gamma\delta \left(\frac{1-\eta^k}{1-\eta}\right),
\end{align*}
where $\eta = 1-\gamma (\xi - \epsilon)$.
\end{theorem}

In order to use this result, you need to bound the 
minimum positive eigenvalue of $G(w)$ for $w\in W\subseteq \mathcal{W}$, and then 
bound the error of the optimal coreset weights $w^\star$ in the sense of \cref{eq:optw_error}.
A notable corollary of \cref{thm:convergence} occurs in the setting where
there exists a $w^\star$ such that
\begin{align*}
\forall \theta\in\Theta, \quad \sum_{m=1}^M w^\star_m f_m(\theta) &= \sum_n f_n(\theta),
\end{align*}
i.e., the optimal coreset is identical to the true posterior distribution, as 
is guaranteed in Statement 2.~of \cref{thm:optimal_kl}.
In this case we can take $\epsilon = \delta = 0$, 
and $\gamma = 1$ to find that
\begin{align*}
\left\|w_{k} - w^\star_k\right\| &\leq (1-\xi)^{k}\left\|w_0 - w^\star_0\right\|.
\end{align*}
This provides intuition about the meaning of \cref{thm:convergence}; as long as 
the optimal coreset posterior is a reasonable approximation to $\pi$, and we use a 
small regularization $\tau>0$ (such that $\xi\approx 1$), then we generally 
need only a very small number of optimization steps to find the optimal coreset.

